Learning Normal Flow Directly From Event Neighborhoods

Event-based motion field estimation is an important task. However, current optical flow methods face challenges: learning-based approaches, often frame-based and relying on CNNs, lack cross-domain transferability, while model-based methods, though more robust, are less accurate. To address the limitations of optical flow estimation, recent works have focused on normal flow, which can be more reliably measured in regions with limited texture or strong edges. However, existing normal flow estimators are predominantly model-based and suffer from high errors. In this paper, we propose a novel supervised point-based method for normal flow estimation that overcomes the limitations of existing event learning-based approaches. Using a local point cloud encoder, our method directly estimates per-event normal flow from raw events, offering multiple unique advantages: 1) It produces temporally and spatially sharp predictions. 2) It supports more diverse data augmentation, such as random rotation, to improve robustness across various domains. 3) It naturally supports uncertainty quantification via ensemble inference, which benefits downstream tasks. 4) It enables training and inference on undistorted data in normalized camera coordinates, improving transferability across cameras. Extensive experiments demonstrate our method achieves better and more consistent performance than state-of-the-art methods when transferred across different datasets. Leveraging this transferability, we train our model on the union of datasets and release it for public use. Finally, we introduce an egomotion solver based on a maximum-margin problem that uses normal flow and IMU to achieve strong performance in challenging scenarios.

==> sec/s31_quasi_optical_flow.tex <==
\begin{definition}[Quasi-Optical Flow]
    Let $\bu\in\R^2$ be an optical flow (OF) vector, then $\bq\in\R^2$ is a quasi-optical flow (QOF) associated with $\bu$ if 
    \begin{equation}
        (\bu-\bq) \cdot \bq = 0
        \label{eqn:quasi_optical_flow}
    \end{equation}
\end{definition}
Eqn. \eqref{eqn:quasi_optical_flow} states that the QOF is the projection of the OF onto an arbitrary direction. So QOF captures one (instead of two) dimension of the OF, and therefore it is named ``quasi''-optical flow. Though we lose one dimension, we obtain the following benefits that outweigh the loss.

Here, three quasi-optical flow vectors associated with an optical flow vector $\bu$ need special attention:

\begin{enumerate}
[leftmargin=21pt]
    \item Optical flow vector $\bu$: $(\bu-\bu)\cdot\bu=0$
    \item Normal flow vector $\bn$: $(\bu-\bn)\cdot\bn=0$.
    \item Zero flow vector $\mathbf{0}$: $(\bu-\mathbf{0})\cdot\mathbf{0}=0$.
\end{enumerate}
All three flow vectors satisfy the definition of quasi-optical flow, which describes three different cases of the neighboring events. As shown in Figure \ref{}, Case 1 happens 

% 

% \noindent\textbf{United Definition of Normal Flow and Optical Flow.}

\noindent\textbf{Predictable from Local Features.}

\noindent\textbf{Useful in Downstreaming Tasks.}

\noindent\textbf{Supervised by Optical Flow.}

==> sec/s36_egomotion_old.tex <==
We demonstrate the usefulness of our normal flow for egomotion estimation. Specifically, we utilize the depth positivity constraint to estimate the translation direction. We assume within a short time interval, we have normalized the event coordinates, per-event normal flow predictions, and we have a rotational velocity read from the IMU sensor. 
%We solve for the translation direction.

\hspace{-2pt}Our egomotion solver uses the depth positivity constraint, which states that all world points are in front of the camera, i.e., have positive depth. Existing methods \cite{fermuller1995passive, barranco2021joint, parameshwara2022diffposenet} utilize this constraint by maximizing the negative depths.
However, when GT normal flow is used, the solution is often not unique because only using the signed direction of the normal flow is a weak constraint. So, when estimated normal flow is used, errors in the estimated normal flow direction determines the location of the minima. Thus we reformulate the problem into a support vector classification (SVC), 
which significantly improves the robustness of the solver.

To define the constraint, denote the magnitude of the normal flow at pixel $\x$ as $n_\x\in\R$, and the direction of the normal flow as $\g_\x\in\R^{2\times 1}$ (with unit norm). We have:
\begin{equation}
    n_\x = \frac{1}{Z_\x}(\g_\x^T A_\x)V + (\g_\x^T B_\x) \Omega \label{eqn:egomotion_constraint}
\end{equation}
where $V\in\R^{3\times1}$ denotes the translation velocity and $\Omega\in\R^{3\times 1}$ denotes the rotational velocity in a small time interval. $Z_\x\in\R$ is the depth of pixel $\x$. $A_\x$ and $B_\x$ are two matrices about the pixel coordinates $\x=(x, y)$:
\begin{align}
\begin{split}
    A_\x=&\left[\begin{matrix}
        -1 & 0 & x \\ 0 & -1 & y
    \end{matrix}\right] \\ 
    B_\x=&\left[\begin{matrix}
        xy & -(x^2+1) & y \\
        (y^2+1) & -xy & -x
    \end{matrix}\right] 
\end{split}
\label{eqn:AB}
\end{align}
By rearranging Eqn. \eqref{eqn:egomotion_constraint}, we obtain
\begin{equation}
    n_\x - (\g_\x^T B_\x) \Omega = \frac{1}{Z_\x}(\g_\x^T A_\x) V
\end{equation}
Since the depth $Z_\x$ is positive, we enforce the following product, denoted as $\rho_\x(V, \Omega)$, to be positive:
\begin{equation}
    \rho_\x(V, \Omega)=\big[(\g_\x^TA_\x) V \big]  \big[n_\x - (\g_\x^T B_\x) \Omega\big] > 0
\end{equation}
\cite{parameshwara2022diffposenet, barranco2021joint} directly solve $\mathrm{min}_{V, \Omega} \mathbb{E}(ReLU(-\rho_x(V, \Omega)))$, but as noted earlier such formulations are sensitive to noise. %the initialization of $V$ and $\Omega$.
%because the solution to the optimization is not unique.

Instead, we formulate the problem into a linear support vector classification problem. Given the rotational estimate, the term $\big(n_\x - (\g_\x^T B_\x) \Omega\big)$ becomes a constant scalar. Therefore, we are solving for $V$ such that $(\g_\x^T A_\x) V$ has a target sign. This becomes a linear binary classification problem, which SVC can solve robustly. The pseudo-code is given below. $p$ is the number of events. $\rA$, $\rB$ are obtained through Eqn. \eqref{eqn:AB}, $\rN$ are the norms of the normal flows, $\rG$ are the directions of normal flows with unit lengths, and $\Omega_0$ is the rotational estimate from the IMU sensor.

\begin{algorithm}
\caption{Egomotion Solver}\label{alg:example}
\begin{algorithmic}[1]
\State \textbf{Input:} $\rA_{p\times 2\times 3}$, $\rB_{p\times 2\times 3}$, $\rN_{p\times 1}$, $\rG_{p\times 2}$, $\Omega_0\in\mathbb{R}^{3\times 1}$.
\State \textbf{Output:} $V\in\mathbb{R}^{3\times 1}$.
\State $Q_{p\times 3} =$ \texttt{batch\_mat\_mul}$(\rG, \rA)$
\State $R_{p\times 1} =$ $\rN - $ \texttt{batch\_mat\_mul}$(\rG, \rB)\times \Omega_0$
\State $Q_{2p\times 3}=$ \texttt{concat($Q$,$-Q$)}
\State $R_{2p\times 1}=$ \texttt{sign(concat($R$,$-R$))}
\State \texttt{svm = LinearSVM(fit\_intercept=False)}
\State $V_{3\times 1} = $\texttt{ svm.fit($Q$,$R$).coef\_}
\State $V = V \:/\: ||V||$
\end{algorithmic}
\end{algorithm}



==> sec/x20_background_of_normal_flow.tex <==
Cornelia will work on this section.
\newpage

==> sec/x43_figures.tex <==









